AMLgentex: Mobilizing Data-Driven Research to Combat Money Laundering

Money laundering enables organized crime by moving illicit funds into the legitimate economy. Although trillions of dollars are laundered each year, detection rates remain low because launderers evade oversight, confirmed cases are rare, and institutions see only fragments of the global transaction network. Since access to real transaction data is tightly restricted, synthetic datasets are essential for developing and evaluating detection methods. However, existing datasets fall short: they often neglect partial observability, temporal dynamics, strategic behavior, uncertain labels, class imbalance, and network-level dependencies. We introduce AMLGentex, an open-source suite for generating realistic, configurable transaction data and benchmarking detection methods. AMLGentex enables systematic evaluation of anti-money laundering systems under conditions that mirror real-world challenges. By releasing multiple country-specific datasets and practical parameter guidance, we aim to empower researchers and practitioners and provide a common foundation for collaboration and progress in combating money laundering.

==> figures/experiments/mid/dist_change.tex <==

\begin{tikzpicture}[scale=0.75]
    \begin{axis}[
        xlabel={overlap},
        ylabel={Avg Precision at Recall > 0.6},
        grid=both,
        xmin=0,
        xmax=1,
        legend style={at={(0.95,0.1)}, anchor=south east},
        ymin = 1e-2,
        ymax = 4e-2
    ]
    
    
    % Plot 1 (no legend)
    \addplot+[] table[x=overlap, y=LogisticRegressor, col sep=comma] {./data/dist_change/testset_average_precision_overlap_nochange.csv};

    \addplot+[] table[x=overlap, y=MLP, col sep=comma] {./data/dist_change/testset_average_precision_overlap_nochange.csv};

    \addplot+[] table[x=overlap, y=GCN, col sep=comma] {./data/dist_change/testset_average_precision_overlap_nochange.csv};

    \addplot+[] table[x=overlap, y=GAT, col sep=comma] {./data/dist_change/testset_average_precision_overlap_nochange.csv};

    \addplot+[] table[x=overlap, y=GraphSAGE, col sep=comma] {./data/dist_change/testset_average_precision_overlap_nochange.csv};


    \end{axis}

\end{tikzpicture}


==> figures/experiments/mid/nodist_change.tex <==

\begin{tikzpicture}[scale=0.75]
    \begin{axis}[
        xlabel={overlap},
        ylabel={Avg Precision at Recall > 0.6},
        grid=both,
        xmin=0,
        xmax=1,
        legend style={at={(0.95,1.1)}, anchor=south west, legend columns=5},
        ymin = 1e-2,
        ymax = 4e-2
    ]


    \addplot+[] table[x=overlap, y=LogisticRegressor, col sep=comma] {./data/dist_change/testset_average_precision_overlap_distchange.csv};
    \addlegendentry{logistic regression}

    \addplot+[] table[x=overlap, y=MLP, col sep=comma] {./data/dist_change/testset_average_precision_overlap_distchange.csv};
    \addlegendentry{MLP}

    \addplot+[] table[x=overlap, y=GCN, col sep=comma] {./data/dist_change/testset_average_precision_overlap_distchange.csv};
    \addlegendentry{GCN}

    \addplot+[] table[x=overlap, y=GAT, col sep=comma] {./data/dist_change/testset_average_precision_overlap_distchange.csv};
    \addlegendentry{GAT}

    \addplot+[] table[x=overlap, y=GraphSAGE, col sep=comma] {./data/dist_change/testset_average_precision_overlap_distchange.csv};
    \addlegendentry{GraphSAGE}

    \end{axis}

\end{tikzpicture}


==> figures/features/no_links.tex <==
\begin{tikzpicture}[scale=0.8, transform shape, >=latex, thick]
    % Nodes
    \node[alertStyle] (a) at (-6,6) {a};
    \node[alertStyle] (b) [below left=1.5cm and 1cm of a] {b};
    \node[nodeStyle] (c) [below=2cm of b] {c};
    \node[nodeStyle] (d) [below right=1.5cm and 1cm of b] {d};
    \node[alertStyle] (f) [above right=0.5cm and 1cm of d] {f};
\end{tikzpicture}

==> figures/features/transductive.tex <==
\begin{tikzpicture}[scale=0.8, transform shape, >=latex, thick]
    % Nodes
    \node[alertStyle] (a) at (-6,6) {a};
    \node[alertStyle] (b) [below left=1.5cm and 1cm of a] {b};
    \node[nodeStyle] (c) [below=2cm of b] {c};
    \node[nodeStyle] (d) [below right=1.5cm and 1cm of b] {d};
    \node[alertStyle] (f) [above right=0.5cm and 1cm of d] {f};
    % Edges (randomly drawn)
    \draw[->, thick, bend right=45] (a) to (b);
    \draw[->, thick] (b) -- (a);
    \draw[->, thick] (a) -- (f);
    \draw[->, thick] (f) -- (b);
    \draw[->, thick] (c) -- (d);
    \draw[->, thick] (b) -- (d);
    \draw[->, thick] (f) -- (d);
\end{tikzpicture}

==> figures/features/transductive_nondir.tex <==
\begin{tikzpicture}[scale=0.8, transform shape, >=latex, thick]
    % Nodes
    \node[alertStyle] (a) at (-6,6) {a};
    \node[alertStyle] (b) [below left=1.5cm and 1cm of a] {b};
    \node[nodeStyle] (c) [below=2cm of b] {c};
    \node[nodeStyle] (d) [below right=1.5cm and 1cm of b] {d};
    \node[alertStyle] (f) [above right=0.5cm and 1cm of d] {f};
    % Edges (randomly drawn)
    \draw[ thick, bend right=45] (a) to (b);
    \draw[thick] (b) -- (a);
    \draw[ thick] (a) -- (f);
    \draw[ thick] (f) -- (b);
    \draw[ thick] (c) -- (d);
    \draw[ thick] (b) -- (d);
    \draw[ thick] (f) -- (d);
\end{tikzpicture}
